NetTAG: A Multimodal RTL-and-Layout-Aligned Netlist Foundation Model via Text-Attributed Graph

Circuit representation learning has shown promise in advancing Electronic Design Automation (EDA) by capturing structural and functional circuit properties for various tasks. Existing pre-trained solutions rely on graph learning with complex functional supervision, such as truth table simulation. However, they only handle simple and-inverter graphs (AIGs), struggling to fully encode other complex gate functionalities. While large language models (LLMs) excel at functional understanding, they lack the structural awareness for flattened netlists. To advance netlist representation learning, we present NetTAG, a netlist foundation model that fuses gate semantics with graph structure, handling diverse gate types and supporting a variety of functional and physical tasks. Moving beyond existing graph-only methods, NetTAG formulates netlists as text-attributed graphs, with gates annotated by symbolic logic expressions and physical characteristics as text attributes. Its multimodal architecture combines an LLM-based text encoder for gate semantics and a graph transformer for global structure. Pre-trained with gate and graph self-supervised objectives and aligned with RTL and layout stages, NetTAG captures comprehensive circuit intrinsics. Experimental results show that NetTAG consistently outperforms each task-specific method on four largely different functional and physical tasks and surpasses state-of-the-art AIG encoders, demonstrating its versatility.

==> section/bak.tex <==
\begin{table}[!t]
% \vspace{-.2in}
\caption{Summary on netlist encoders with pretrain-finetune paradigm.}
% \vspace{-.15in}
\resizebox{0.5\textwidth}{!}{

\begin{tabular}{c||c|c|c|c}
\toprule
\textbf{Method} & \textbf{Cell Type}   & \textbf{Circuit}       & \textbf{Modality}      & \textbf{Task}         \\ \hline \hline
DeepGate~\cite{li2022deepgate}        & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}AND,\\      INV\end{tabular}} & \multirow{4}{*}{Combinational} & \multirow{5}{*}{Graph} & \multirow{5}{*}{Functional} \\
DeepGate2~\cite{shi2023deepgate2}       &                      &                        &                        &                       \\
DeepGate3~\cite{shi2024deepgate3}       &                      &                        &                        &                       \\
FGNN~\cite{wang2022functionality, wang2024fgnn2}            &                      &                        &                        &                       \\ \cline{3-3}
DeepSeq~\cite{khan2024deepseq}$^\star$         &                      & Sequential                   &                        &                       \\ \hline 
\textbf{NetEncoder}      & \textbf{Any Gate}       & \textbf{Comb.+Seq.}             & \textbf{Text+Graph}           & \textbf{Func+Phys}     \\ \bottomrule      
\end{tabular}


}

\begin{tablenotes}\footnotesize
\item $^\star$ DeepSeq predicts netlist gate toggle rate to estimate power consumption, rather than directly modeling power.
\end{tablenotes} 

\label{tbl:works}
\vspace{-.1in}
\end{table}




\begin{table*}[!t]
\centering
\caption{Summary on netlist encoders with pretrain-finetune paradigm.}
% \vspace{-.15in}
\resizebox{0.9\textwidth}{!}{

\begin{tabular}{c||cc|ccc|cc} \toprule
\multirow{2}{*}{\textbf{Method}}                   & \multicolumn{2}{c|}{\textbf{Target Circuit}}                                                                                                                  & \multicolumn{3}{c|}{\textbf{Encoding Method}}                                                                                                                                                                         & \multicolumn{2}{c}{\textbf{Downstream Tasks}}                                                                                                                           \\ \cline{2-8}
                                                   & Cell Type                                                                & Circuit Type                                                                      & Modality                                                            & Pre-Train Target                                                    & Corss-Stage Align                                                   & Target                                                                              & Type                                                                         \\ \hline \hline
DeepGate~\cite{li2022deepgate}                     & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}AND,\\      INV\end{tabular}} & Comb.                                                   & \multirow{5}{*}{Graph}                                              & Gate                                                                     & \multirow{5}{*}{N/A}                                                & \multirow{5}{*}{Gate}                                                                    & \multirow{5}{*}{Functional}                                                  \\
DeepGate2~\cite{shi2023deepgate2}                  &                                                                          &  Comb.                                                                                 &                                                                     & Gate                                                                     &                                                                     &                                                                                          &                                                                              \\
DeepGate3~\cite{shi2024deepgate3}                  &                                                                          &  Comb.                                                                                 &                                                                     & Gate+Circuit                                                             &                                                                     &                                                                                          &                                                                              \\
FGNN~\cite{wang2022functionality,   wang2024fgnn2} &                                                                          & Comb.                                                                                  &                                                                     & Gate                                                                     &                                                                     &                                                                                          &                                                                              \\
DeepSeq~\cite{khan2024deepseq}$^\star$             &                                                                          & Seq.                                                                        &                                                                     & Gate                                                                     &                                                                     &                                                                                          &                                                                              \\ \hline

\textbf{NetEncoder}                                                      &  \textbf{\begin{tabular}[c]{@{}c@{}}Arbitrary\\      Gate\end{tabular}}                                                 & \textbf{\begin{tabular}[c]{@{}c@{}}Comb.\&\\      Seq.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text\&\\      Graph\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gate\&\\      Reg. Cone\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RTL\&\\      Layout\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gate\&\\      Reg. Cone\&\\      Circuit\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Functional\&\\      Physical\end{tabular}} \\ \bottomrule


\end{tabular}


}

\begin{tablenotes}\footnotesize
\item $^\star$ DeepSeq predicts netlist gate toggle rate to estimate power consumption, rather than directly modeling power.
\end{tablenotes} 

\label{tbl:works}
\vspace{-.1in}
\end{table*}
